Multi-source adversarial transfer learning based on similar source domains with local features

Transfer learning leverages knowledge from other domains and has been successful in many applications. Transfer learning methods rely on the overall similarity of the source and target domains. However, in some cases, it is impossible to provide an overall similar source domain, and only some source domains with similar local features can be provided. Can transfer learning be achieved? In this regard, we propose a multi-source adversarial transfer learning method based on local feature similarity to the source domain to handle transfer scenarios where the source and target domains have only local similarities. This method extracts transferable local features between a single source domain and the target domain through a sub-network. Specifically, the feature extractor of the sub-network is induced by the domain discriminator to learn transferable knowledge between the source domain and the target domain. The extracted features are then weighted by an attention module to suppress non-transferable local features while enhancing transferable local features. In order to ensure that the data from the target domain in different sub-networks in the same batch is exactly the same, we designed a multi-source domain independent strategy to provide the possibility for later local feature fusion to complete the key features required. In order to verify the effectiveness of the method, we made the dataset "Local Carvana Image Masking Dataset". Applying the proposed method to the image segmentation task of the proposed dataset achieves better transfer performance than other multi-source transfer learning methods. It is shown that the designed transfer learning method is feasible for transfer scenarios where the source and target domains have only local similarities.

==> chapters/authors.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a1.png}}]{First A. Author} (M'76--SM'81--F'87) and all authors may include 
	biographies. Biographies are often not included in conference-related
	papers. This author became a Member (M) of IEEE in 1976, a Senior
	Member (SM) in 1981, and a Fellow (F) in 1987. The first paragraph may
	contain a place and/or date of birth (list place, then date). Next,
	the author's educational background is listed. The degrees should be
	listed with type of degree in what field, which institution, city,
	state, and country, and year the degree was earned. The author's major
	field of study should be lower-cased. 
	
	The second paragraph uses the pronoun of the person (he or she) and not the 
	author's last name. It lists military and work experience, including summer 
	and fellowship jobs. Job titles are capitalized. The current job must have a 
	location; previous positions may be listed 
	without one. Information concerning previous publications may be included. 
	Try not to list more than three books or published articles. The format for 
	listing publishers of a book within the biography is: title of book 
	(publisher name, year) similar to a reference. Current and previous research 
	interests end the paragraph. The third paragraph begins with the author's 
	title and last name (e.g., Dr.\ Smith, Prof.\ Jones, Mr.\ Kajor, Ms.\ Hunter). 
	List any memberships in professional societies other than the IEEE. Finally, 
	list any awards and work for IEEE committees and publications. If a 
	photograph is provided, it should be of good quality, and 
	professional-looking. Following are two examples of an author's biography.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a2.png}}]{Second B. Author} was born in Greenwich Village, New York, NY, USA in 
	1977. He received the B.S. and M.S. degrees in aerospace engineering from 
	the University of Virginia, Charlottesville, in 2001 and the Ph.D. degree in 
	mechanical engineering from Drexel University, Philadelphia, PA, in 2008.
	
	From 2001 to 2004, he was a Research Assistant with the Princeton Plasma 
	Physics Laboratory. Since 2009, he has been an Assistant Professor with the 
	Mechanical Engineering Department, Texas A{\&}M University, College Station. 
	He is the author of three books, more than 150 articles, and more than 70 
	inventions. His research interests include high-pressure and high-density 
	nonthermal plasma discharge processes and applications, microscale plasma 
	discharges, discharges in liquids, spectroscopic diagnostics, plasma 
	propulsion, and innovation plasma applications. He is an Associate Editor of 
	the journal \emph{Earth, Moon, Planets}, and holds two patents. 
	
	Dr. Author was a recipient of the International Association of Geomagnetism 
	and Aeronomy Young Scientist Award for Excellence in 2008, and the IEEE 
	Electromagnetic Compatibility Society Best Symposium Paper Award in 2011. 
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{a3.png}}]{Third C. Author, Jr.} (M'87) received the B.S. degree in mechanical 
	engineering from National Chung Cheng University, Chiayi, Taiwan, in 2004 
	and the M.S. degree in mechanical engineering from National Tsing Hua 
	University, Hsinchu, Taiwan, in 2006. He is currently pursuing the Ph.D. 
	degree in mechanical engineering at Texas A{\&}M University, College 
	Station, TX, USA.
	
	From 2008 to 2009, he was a Research Assistant with the Institute of 
	Physics, Academia Sinica, Tapei, Taiwan. His research interest includes the 
	development of surface processing and biological/medical treatment 
	techniques using nonthermal atmospheric pressure plasmas, fundamental study 
	of plasma sources, and fabrication of micro- or nanostructured surfaces. 
	
	Mr. Author's awards and honors include the Frew Fellowship (Australian 
	Academy of Science), the I. I. Rabi Prize (APS), the European Frequency and 
	Time Forum Award, the Carl Zeiss Research Award, the William F. Meggers 
	Award and the Adolph Lomb Medal (OSA).
\end{IEEEbiography}

==> chapters/reference.tex <==
%\newpage
\bibliography{wpref}

==> chapters/related_work.tex <==
\section{RELATED WORK}
\subsection{Multi-source transfer learning}

\par
Different from these works, our work pays more attention to the complementary local features between each source domain. In the face of a scene where there is no global similarity to the source domain, how to mine local common features from multiple source domains with limited global similarity and integrate them to improve the task performance of the target domain is a problem we need to solve.
\subsection{Attention Mechanism}
As we all know, the human attention mechanism not only pays attention to the whole object, but also pays more attention to the local useful information of the object. Inspired by the human attention mechanism, some works that introduce the attention mechanism make it possible to mine and enhance the local features of objects, so that important features can be distinguished from insignificant features. For example\cite{RN68} apply separate attention clusters to different feature sets and then concatenate the outputs for classification. We argue that the idea of distinguishing whether local features are important is necessary for domain adaptation, especially when each source domain has only some similar local features. Because the transferability of different local features is different for the same domain, we should distinguish transferable and non-transferable local features, such as assigning greater weight to important local features.

==> tables/experiments_setting.tex <==
\begin{table}[]
	%\centering
	%\tiny
	% \footnotesize  %此处写字体大小控制命令
	\caption{Experiments settings}   
	\label{experiments_setting}
	\begin{tabular}{cccccc}
		\hline
		\multicolumn{2}{c}{Name}                  & Target & Source 1 & Source 2 & Method                        \\ \hline
		\multirow{3}{*}{Adversarial:} & 2 Sources & \checkmark      & \checkmark        & \checkmark        & ATL$^a$ \\
		& Source 1  & \checkmark      & \checkmark        &          & ATL \\
		& Source 2  & \checkmark      &          & \checkmark        & ATL \\ \hdashline[1pt/1pt]
		\multirow{3}{*}{Ablation:}    & 2 Sources & \checkmark      & \checkmark        & \checkmark        & MTL$^b$           \\
		& Source 1  & \checkmark      & \checkmark        &          & MTL           \\
		& Source 2  & \checkmark      &          & \checkmark        & MTL           \\ \hdashline[1pt/1pt]
		\multicolumn{2}{c}{Only Target}           & \checkmark      &          &          & DL$^c$                 \\ \hline
	\end{tabular}\\
\footnotesize{$^a$ ATL $=$ Adversarial Transfer Learning}\\
\footnotesize{$^b$ ML $=$ Multi-task Learning}\\
\footnotesize{$^c$ DL $=$ Deep Learning}
\end{table}

==> tables/table_net_struct.tex <==
\begin{table}[]
	\caption{The structure definition of each layer in the network structure}   
	\label{table_net_struct}
\begin{tabular}{ccccc}
\hline
Structure               & Layer type & F/S$^a$ & P/S$^b$ & A/U$^c$      \\ \hline
\multirow{3}{*}{Down}   & MaxPool2d  & 2×2 & -   & - \\
& Conv2d     & 3×3 & 1   & ReLU     \\
& Conv2d     & 3×3 & 1   & ReLU     \\ \hdashline[1pt/1pt]
\multirow{3}{*}{Up}     & Upsample   & -   & 2   & Bilinear \\
& Conv2d     & 3×3 & 1   & ReLU     \\
& Conv2d     & 3×3 & 1   & ReLU     \\ \hdashline[1pt/1pt]
Fc & Linear     & -   & -   & ReLU     \\ \hline
\end{tabular}\\
\footnotesize{$^a$ F/S $=$ Filter/Stride\ size}\\
\footnotesize{$^b$ P/S $=$ Padding / Scale\ factor}\\
\footnotesize{$^c$ A/U $=$ Activation function / Upsampling algorithm}
\end{table}
